Qubit error bursts in superconducting quantum processors of Quantum Inspire: quasiparticle pumping and anomalous time dependence

We investigate qubit error bursts in 5- and 7-transmon processors of similar design, fabrication and packaging, but with different types of qubit Josephson junctions. Measurements for each are performed in two refrigerators to discern device-specific from refrigerator-dependent characteristics. The duration and rate of bursts are device specific but within the range of prior experiments and consistent with ionizing radiation. We observe two unforeseen signatures specifically in the processor with Dolan junctions. First, increasing the rate of $\pi$ pulsing in the detection scheme shortens the recovery time to equilibrium, which is explained by a quasiparticle pumping mechanism. The second signature is an anomalous time dependence in the burst rate: a surge happens days or weeks after cooldown, followed by a strong suppression that persists until thermal cycling.

==> Uploaded/sections/Discussion.tex <==

In summary, we have investigated qubit error bursts in the 5- and 7-transmon processors made available (at different times) via the Quantum Inspire platform.
We use a detection scheme exploiting mid-circuit measurement and signal-processing passes to discern real bursts from false positives due to baseline $\Tone$ and readout errors, despite the low qubit count.
$\Sfive$ and $\Sseven$ exhibit refrigerator-independent burst rates $\gammakept \sim 1.5$ and $1~\minutes^{-1}$, respectively, comparable to those reported in Refs.~\cite{McEwen22, Harrington24, McEwen24} after accounting for device dimensions.
The processors reveal more differences that are interesting in view of the similarity in processor design, fabrication and packaging.
First, the recovery time of bursts is also refrigerator independent and differs by a factor $\times 8$, possibly due to difference in JJ electrode geometries. Second,  $\trec$ in $\Sfive$ can be shortened by increasing the rate of applied $\pi$ pulses in the detection scheme. This is a manifestation of QP pumping away from the transmon JJ into a nearby QP trap created by the Dolan-bridge JJ fabrication process. Such pumping is not possible in $\Sseven$ as its Manhattan-style JJs lack such built-in trap. Third, $\Sfive$ shows an anomalous surge and subsequent reduction of $\gammakept$, with some refrigerator-dependent characteristics. Given the obvious benefit to QEC of limiting the rate, duration and globality of qubit error bursts, understanding the physics of the surge and its aftermath motivates further research.




==> Uploaded/sections/Introduction.tex <==
It is counterintuitive that high-energy radiation of cosmogenic origin and from local radioactivity, with as much as MeV-GeV per particle/photon, can cause the majority of qubits in a superconducting quantum processor to lose energy~\cite{McEwen22, McEwen24, Harrington24, Li24}. Yet, the various energy inter-conversion processes underlying this catastrophic effect are understood~\cite{Martinis21, Kaplan76}. Incident radiation sheds up to MeV in the form of phonons and substrate electron-hole pairs, with most of the latter quickly recombining to produce more phonons. Carrying $\sim90\%$ of the shed energy, phonons proliferate by frequency down-conversion and propagate across the substrate, partially transmitting into superconducting layers where they break Cooper pairs into quasiparticles (QPs). Through their continued interactions, phonons and QPs down-convert in a process culminating with $\sim60\%$ of the initial phonon energy as QPs with energy close to the superconducting gap $\Delta$ and the rest as phonons with energy $<2\Delta$. QPs on the electrodes of qubit Josephson junctions (JJs) can tunnel across by absorbing the qubit transition energy $\fq$~\cite{Martinis09, Catelani11}. Such qubit relaxation errors persist until the QP density near qubit JJs subsides through recombination and trapping mechanisms. However, $2\Delta$ phonons produced by recombination of QPs can re-break Cooper pairs, increasing the recovery time. Ultimately, most of the energy imparted by the radiation escapes the processor as $\leq2\Delta$ phonons via interconnects (AlSi wirebonds, In bumps, etc.) and clamping points.

The increased propensity for qubits to relax, made global by phonon propagation, is a source of correlated errors and consequently problematic for quantum error correction (QEC) and eventually fault-tolerant quantum computing. In fact, such error bursts already set the performance limit of state-of-the-art QEC experiments~\cite{Google21, Google25}. Several strategies are being pursued that can help mitigate the impact. Recent large-scale efforts involve moving experimental setups to deep underground facilities to reduce the flux of ionizing radiation of cosmogenic origin~\cite{Cardani21, Gusenkova22}. Device-level innovations include phonon traps~\cite{Patel17, Henriques19, DeVisser21, Bargerbos23}, substrate etching to block phonon propagation~\cite{Chu16, Rostem18, Karatsu19}, backside metallization to enhance phonon downconversion~\cite{Iaia22, Yelton24, Larson25}, QP traps using normal and low-gap superconductors~\cite{Riwar16, Riwar19, Martinis21, Pan22, Thorbeck23}, and band-gap engineering of JJ electrodes~\cite{Diamond22, kamenov23, Connolly24, McEwen24, kurilovich25, Nho26}. These innovations are often assessed not by their impact on the rate or recovery dynamics of qubit error bursts but on the average QP density in qubit JJ electrodes, extracted by measuring QP tunneling rates~\cite{Riste13}. Some experiments observe exponential or power-law time dependence of QP tunneling rates after cooldown~\cite{Mannila22, Anthony24, Yelton25, kerschbaum26}, attributed to gradual thermalization of substrates, metal films, device packaging, and shielding.

In this Letter, we investigate qubit error bursts in two transmon-based processors of Quantum Inspire~\cite{QI_website}, Starmon-5 (henceforth $\Sfive$) and Starmon-7 ($\Sseven$), with similar design, fabrication and packaging but different Al/AlOx/Al JJ types (Dolan~\cite{Dolan77} versus Manhattan~\cite{Potts01}, respectively). We extract the rate (with and without lead shielding) and duration of bursts in each device in two dilution refrigerators (A and B) to discern device-specific from refrigerator-dependent characteristics. The rate and duration of error bursts are device specific and within the range reported by prior experiments. However, we observe two unforeseen signatures only in $\Sfive$. First, the duration of bursts is shortened by increasing the rate of qubit $\pi$ pulsing in two variants of the detection scheme. We explain this effect as a pulse-induced QP pumping mechanism possible only in the Dolan-bridge JJs, whose fabrication produces a built-in QP trap. The second signature is an anomalous time dependence in the error burst rate: after holding steady for days or weeks since cooldown, the rate  surges by one to two orders of magnitude for several hours and then gradually decreases over days to a value two orders of magnitude lower than immediately post-cooldown, persisting until a thermal cycle. The physical mechanism for this anomalous time dependence remains unclear, inviting suggestions. The vanishing of the burst rate post-surge could be exploited to mitigate radiation-induced correlated errors.


==> Uploaded/sections/Other_stuff.tex <==
\section{Acknowledgements}
We thank J.~Baselmans, K.~Karatsu, C.~Andersen, B.~Plourde, L.~Kouwenhoven, G.~Frossati, and their teams for helpful discussions; S.~van der Meer and M.~Sarsby for assistance with dilution
refrigerators; G.~Calusine and W.~Oliver for providing traveling-wave parametric amplifiers; the TU Delft Reactor Institute for the lead shield;
the Kavli Nanolab Delft staff for cleanroom support; and V.~Sinha for project management assistance.
This research is funded by the Dutch National Growth Funds and Quantum Delta NL (KAT-1 StartImpulse and Phase 2), the European Union Flagship on Quantum Technology (OpenSuperQplus100, No. 101113946), Intel Corporation,  the Dutch Ministry of Economic Affairs [Allowance for Top Consortia for Knowledge and Innovation (TKI)], and the Netherlands Organization for Scientific Research (NWA.1292.19.194). M.S. acknowledges funding from the Google PhD fellowship program.

\section{Authors Contribution}
G.R.D.C., M.S., J.F.M., and L.D.C conceptualized the experiment.
G.R.D.C. and M.S. performed the experiment and data analysis.
J.F.M. performed initial experiments.
N.M. fabricated $\Sfive$, A.K. and M.F. fabricated $\Sseven$.
M.B., N.H. and L.D.C. designed the two processors.
M.S.M. implemented mid-circuit measurement and B.S. developed monitoring software in Quantum Inspire.
S.V.S. performed post-fabrication trimming of $\Sseven$ resonators.
G.R.D.C., M.S. and L.D.C. wrote the manuscript with feedback from coauthors.
L.D.C. supervised the project.
G.R.D.C. and M.S. contributed equally to this work.

\section{Competing Interests}
The authors declare no competing interests.

\section{Data Availability}
All data shown are available at \url{https://github.com/DiCarloLab-Delft/QubitErrorBursts}.
Further materials can be provided upon request. 

==> Uploaded/sections/Results.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=\columnwidth]{figures/Figure_1.png}
\caption{
Detection and characterization of simultaneous error events.
(a) Repeated detection subcircuit described in the main text. Blocks labelled $W$ correspond to idling (waiting) periods.
(b,c) Average of kept and rejected events for (b) $\Sfive$ ($\tcycle=100~\us$, $\nth=5$) and (c) $\Sseven$
($\tcycle=10~\us$, $\nth=7$). Note the different timescales on horizontal axes. For kept events in $\Sfive$ ($\Sseven$), the baseline is fully recovered in $\trec \sim 2~\ms$ $(\sim250~\us)$.
(d) Cumulative sum of kept events for $\Sfive$ ($\Sseven$) for $\nth=3$ and maximized $\nth=5$ $(7)$.
(e) Extracted rate of kept events $\gammakept$ as a function of $\nth$ for both processors.
}
\label{fig:Figure1}
\end{figure}

The burst detection scheme [Fig.~\ref{fig:Figure1}(a)] consists of back-to-back repetitions of the following subcircuit: all qubits are $\pi$ pulsed in $\tx=20~\ns$, idled for $\twait=2~\us$, readout in $\tro$, and
idled again for $\tidle$, for a total subcircuit duration
$\tcycle = \tx + \twait + \tro + \tidle$ [$\tro=2~(1)~\us$ in $\Sfive~(\Sseven)$]. Later, we vary $\tcycle$ through $\tidle$.
The string of measurement outcomes for each qubit is ideally a series of alternating 0s and 1s.
We define a qubit error as two consecutive 0 outcomes.
We do not consider two consecutive 1 outcomes as an error because leakage to the second-excited state, which can be residually induced by measurement, produces this signature as well. We define a simultaneous error event whenever the number of qubits in error $n$ peaks at $n\geq \nth$, with $\nth$ a set event threshold.


To distinguish bursts originating from ionizing radiation from error events caused by the baseline qubit relaxation time $\Tone$ and readout ($\RO$) errors~\cite{SOM_CR}, we post-process the time series of $n$ using two passes.
The first marks all simultaneous events using the $n\geq \nth$ condition. The second pass separates events based on their duration.
For bursts induced by ionizing radiation, the characteristic time $\trec$ for $n$ to fully return to the baseline varies widely across reported experiments,
from $\sim 150~\us$~\cite{Li24} to $\sim 100~\ms$~\cite{McEwen22}. For error events triggered by baseline $\Tone$ and $\RO$ errors, the baseline is recovered in just $\sim 2 \tcycle$. Therefore, a large separation of scales between $\tcycle$ and $\trec$ is best for discrimination.
The second pass uses template matching following Refs.~\cite{McEwen22, Wu25}, with a stepped exponential decay template function (see~\cite{SOM_CR}).
We use the peak value of the matched-filter output to set the start ($t=0$) of each event, which is used when averaging over events.
We manually optimize the template function decay constant to best separate the two apparent distributions in the histogram of peak output values.
As $\nth$ increases, the edge of the distribution associated with events caused by baseline $\Tone$ and RO errors (which we aim to reject) shifts to lower values [see Fig.~\ref{fig:cr_filtering}(d) in~\cite{SOM_CR}]. We therefore set the threshold for keeping and rejecting events at $\nth=3$ to minimize false positives, and apply this same threshold for all cases with $\nth>3$.

We first estimate $\trec$ in the two processors by averaging the time series of $n$ for kept events.  For $\Sfive$~$(\Sseven$), we use $\tcycle=100~(10)~\us$ and set $\nth=5~(7)$ to maximize signal range. We find $\trec\sim2~\ms$ for $\Sfive$ and $\sim250~\us$ for $\Sseven$. This $\times8$ difference is device specific, as confirmed by repeating measurements for each device in refrigerator B (see Fig.~\ref{fig:FigKeptFridges} in~\cite{SOM_CR}). Furthermore, we have also found that $\trec$ is robust to variations in packaging. For example, doubling the density of ground-plane wirebonds in $\Sseven$ to roughly match that in $\Sfive$ did not further shorten its $\trec$. In $\Sfive$, adding small amounts of GE varnish to the backside corners of the substrate to improve thermal contact and clamping (which $\Sseven$ has) also did not shorten its $\trec$. We speculate that the difference in $\trec$ between the processors may instead be rooted in geometrical differences between their JJ electrodes (see~\cite{SOM_CR} for images). Effective QP trapping and recombination rates vary by more than one order of magnitude in the literature (see~\cite{Wang14, Derooij21} and references therein) and are known to depend on electrode geometry. Detailed modeling beyond our present capabilities is required to substantiate this.

\begin{figure}[ht]
\centering
\includegraphics[width=\columnwidth]{figures/Figure_2.png}
\caption{
Signature of QP pumping in $\Sfive$ and absence thereof in $\Sseven$.
(a) Variant of the repeated detection subcircuit: an even number $m$ of $\pi$ pulses is inserted after readout.
(b,c) Average of kept events for (b) $\Sfive$ and (c) $\Sseven$ with fixed $m=0$ and varying $\tcycle$. $\Sfive$ shows an increase in $\trec$ as $\tcycle$
increases from $10$ to $100~\us$. $\Sseven$ does not show any such dependence.
(d,e) Average of kept events for (c) $\Sfive$ and (d) $\Sseven$ with fixed $\tcycle=100$ and $30~\us$, respectively, but increasing $m$.
In $\Sfive$, but not in $\Sseven$, $\trec$ decreases as $m$ increases from 0 to 6. In combination, these results demonstrate that increasing the net rate of $\pi$ pulses
in the detection scheme shortens $\trec$ in $\Sfive$.
}
\label{fig:Figure2}
\end{figure}

\begin{figure}[ht]
\centering
\includegraphics[width=\columnwidth]{figures/Figure_3.png}
\caption{
Schematics of the transmon Josephson junctions of $\Sfive$ fabricated using the Dolan-bridge technique.
(a) Top view. (b) Cross section along the long axis. (c) Energy diagram illustrating the superconducting energy gaps $\DeltaAl$ in the thin (bottom) and
thick (top) Al layers deposited by double-angle evaporation. The difference between these gaps $\delta \DeltaSfive$ is smaller than the qubit transition energy $h \fq$ in each transmon.
[The much larger gap of the NbTiN transmon capacitor pads $(\Delta_{\mathrm{NbTiN}}\sim2.3~\mathrm{meV})$ is not shown.]  With the qubit in $\ket{1}$, a QP on the thick left layer can tunnel across the dominant JJ into the thin right layer by relaxing the qubit to $\ket{0}$, then diffuse and tunnel onto the thick right layer, where it becomes trapped. A subsequent $\pi$ pulse re-excites the qubit, commencing another cycle of QP pumping to the trap.
}\label{fig:Figure3}
\end{figure}

Having characterized their recovery time, we next turn to the frequency of bursts. The rate of kept events $\gammakept$ is extracted from $\sim 4~\hours$ of acquisition time (not wall-clock time) for each processor.
In $\Sfive$, we observe $\gammakept = 1/(38.9\pm2.1~\s)$ at $\nth=3$ [Fig.~\ref{fig:Figure1}(d)]. We can compare this rate to the known muon flux at sea level~\cite{Cecchini12}, approximately $1~\cm^{-2}\minutes^{-1}$, and thus $1/(90~\s)$ for the $8~\mm \times 8~\mm$ area common to both processors.
In $\Sseven$, we observe $\gammakept = 1/(58.9\pm3.8~\s)$ at $k=3$ [Fig.~\ref{fig:Figure1}(e)]. It is possible that the lower $\gammakept$ may be due to a higher rate of false rejects in $\Sseven$ resulting from the short $\trec$. We can compare these rates to reported values in experiments~\cite{McEwen22, Harrington24, McEwen24} that use similar detection schemes. Accounting for device dimensions (see~\cref{tab:TableRates}) shows  that $\gammakept$ in $\Sfive$ is comparable to that in Ref.~\cite{Harrington24},
while $\gammakept$ in $\Sseven$ is comparable to those in Refs.~\cite{McEwen22, McEwen24}. Figure~1(e) shows the dependence of $\gammakept$ on $\nth$, revealing that the majority of bursts affect the majority of qubits in each device.

Varying $\tcycle$ reveals a more striking difference between $\Sfive$ and $\Sseven$ that connects to the different types of JJ used for their transmons (Fig.~\ref{fig:Figure2}). In $\Sfive$, varying $\tcycle$ from $100$ to $10~\us$ does not affect $\gammakept~(\nth=3)$~\cite{SOM_CR}, but decreases $\trec$ from $\sim2~\ms$ to $\sim500~\us$. In sharp contrast, no change in $\trec$ is
observed in $\Sseven$ over the same $\tcycle$ range (no data shown for $\tcycle=100~\us$).
A similar effect is observed in a variant of the detection subcircuit where, keeping $\tcycle=100~(30)~\us$ for $\Sfive$ $(\Sseven)$, we insert an even number $m$ of $\pi$ pulses during $\tidle$. Again, $\trec$ decreases monotonically with increasing $m$ for $\Sfive$, but not $\Sseven$.

\begin{figure*}[ht]
\centering
\includegraphics[width=\textwidth]{figures/Figure_4.png}
\caption{
Example observation of the surge in $\Sfive$ while in refrigerator A.
(a) Cumulative sum of kept events (left axis) and average $\Tone$ (right) as a function of elapsed time at base temperature (bottom) and elapsed time running the detection circuit of Fig.~\ref{fig:Figure1}(a) ($\tcycle=30~\us$, $\nth=3$).
After 26 days at base temperature with similar characteristics as Fig.~\ref{fig:Figure1}, $\gammakept$ suddenly surges by a factor $\sim\times10$ and average $\Tone$ drops by $\sim\times3$. Over the next several days, $\gammakept$ monotonically decreases, ultimately settling to a value $\sim \times 100$ lower than at the start of the experiment, and average $\Tone$ gradually recovers.
(b) Average of kept events ($\tcycle=30~\us$, $\nth=5$) over the full observation period.
We use a second pass of template matching (see~\cite{SOM_CR}) to discern $37$ bursts with atypically long recovery times (red), all of which are detected at the onset of the surge. See~\cite{SOM_CR} for other observations of the surge showing some refrigerator-specific characteristics.
See~\cite{SOM_CR} for other observations of the surge in $\Sfive$.
}
\label{fig:Figure4}
\end{figure*}

To understand why the net rate of $\pi$ pulses in the detection scheme affects $\trec$ in $\Sfive$, recall that a prior experiment~\cite{Gustavsson16} has shown active reduction of QP densities near active qubit JJs through repeated $\pi$ pulsing. QP pumping, as the effect is known, was first evidenced as pulse-controlled enhancement of $\Tone$ in a flux qubit.
Here, the effect is evidenced as a pulse-controlled reduction of $\trec$ in $\Sfive$. The reason becomes clear upon noting that Dolan-bridge JJs like those of $\Sfive$ have a built-in QP trap (Fig.~\ref{fig:Figure3}), while
Manhattan-style JJs like those of $\Sseven$ do not (see Fig.~\ref{fig:FigDevices}).

Our Dolan JJs are defined by double-angle evaporation of Al layers with intermediate oxidation~\cite{Muthusubramanian24}, with bottom (top)
layer thickness $d=30~(60)~\nm$. The cross-section schematic in Fig.~\ref{fig:Figure3}(b) shows the dominant active JJ near the center, which has the smallest overlap area
and is largely responsible for setting the qubit transition frequency $\fq$. There are two more JJs  created by the shadowing mechanism: a large active one to the left and another large inactive one to the right.

Owing to their different $d$, the bottom and top layers are expected to have different superconducting gap $\DeltaAl$.
For thin Al films, $\DeltaAl$ increases with decreasing $d$. Using the empirical model~\cite{Marchegiani22}
\[
\DeltaAl(d) = \DeltaBulk + \alpha/d
\]
with $\DeltaBulk = 180~\ueV$ and $\alpha = 600~\ueV \cdot \nm$, we estimate a gap difference between the layers
$\delta \DeltaSfive \sim h \times 2.4~\GHz$. As $h \fq > \delta \DeltaSfive$ for all its  transmons, we do not expect band-gap engineering effects~\cite{Diamond22, kamenov23, Connolly24, McEwen24, kurilovich25, Nho26} to play a role in $\Sfive$.

During a burst, if the qubit is in the first-excited state $(\ket{1})$, a QP at the band edge of the thick layer on the left can tunnel across the dominant JJ
onto the thin layer on the right by absorbing the qubit energy (i.e., relaxing the qubit to the ground state $\ket{0}$). The QP can then diffuse rightward, tunnel across to the thick layer on the right, and drop to the band edge, becoming trapped [Fig.~\ref{fig:Figure3}(c)].  In this way, repeated qubit re-excitation by $\pi$ pulses creates a net pumping of QPs away from the thick layer to the left of the dominant JJ to the trap on the right. This pumping process shortens $\trec$.

Finally, we report another phenomenon observed only in $\Sfive$ but for which we currently lack explanation, inviting suggestions from the community.
The phenomenon is an anomalous time dependence in $\gammakept$ that is best described as a surge. We do not find any link between this surge and any sudden change in any pressure or temperature within the refrigerator or any applied microwave-frequency or baseband pulsing. Figure~\ref{fig:Figure4} presents a typical observation in refrigerator A
for $\tcycle=30~\us$.
After 3-4 weeks at base temperature showing a steady value, $\gammakept$ surges by an order of magnitude, accompanied by
a sharp decrease in average $\Tone$. During this surge, some kept events show uncharacteristically long $\trec~\sim3~\ms$. Over the next few days, $\gammakept$ decreases
monotonically and ultimately settles to a value $\sim\times100$ lower than at the start of the experiment. In parallel, the average $\Tone$ gradually recovers to pre-surge values.
The almost vanishing $\gammakept$ persists until thermal cycling. We have performed cycles to $4~\K$ as well as to room temperature, finding that $\gammakept$ fully resets
in both cases.
The surge observed in $\Sfive$ has some refrigerator-specific characteristics. In refrigerator A, the surge has occured in all 4 cooldowns since it was first identified,
with the characteristics described above (see~\cite{SOM_CR} for more observations). In refrigerator B, the surge has been observed in $12$ out of $20$ cooldowns. In 11 of
them, the surge began just $\sim1$ day after reaching base temperature, and after $\sim1$ week in the other. The onset is marked by an increase in $\gammakept$ by
$\sim\times100$, i.e., even stronger than in refrigerator A. Cooldowns during which the surge did not occur have maintained base temperature for periods ranging between
$4$ and $42$ days. Curiously, the surge has not been observed in any of 4 cooldowns since adding GE varnish to the backside of $\Sfive$. This is noteworthy as $\Sseven$,
which has had such GE varnish from the beginning, has not shown any surge in either refrigerator to date. However, more cooldowns are required to establish
causality.

Equally intriguing as the trigger source for the surge is the physical mechanism causing $\gammakept$ to practically vanish in the days following. Evidently, no significant time dependence is known to occur in the incidence rate of ionizing radiation of cosmogenic origin (or local radioactivity in our lab). Rather, some on-chip mechanism must be at play.



==> Uploaded/sections/authors.tex <==
\author{G.~R.~Di~Carlo}
\thanks{These authors contributed equally to this work.}
\affiliation{QuTech and Kavli Institute of Nanoscience, Delft University of Technology, P.O. Box 5046, 2600 GA Delft, The Netherlands}

\author{M.~Samiotis}
\thanks{These authors contributed equally to this work.}
\affiliation{QuTech and Kavli Institute of Nanoscience, Delft University of Technology, P.O. Box 5046, 2600 GA Delft, The Netherlands}

\author{A.~Kamlapure}
\affiliation{QuTech and Kavli Institute of Nanoscience, Delft University of Technology, P.O. Box 5046, 2600 GA Delft, The Netherlands}

\author{M.~Finkel}
\affiliation{QuTech and Kavli Institute of Nanoscience, Delft University of Technology, P.O. Box 5046, 2600 GA Delft, The Netherlands}

\author{N.~Muthusubramanian}
\affiliation{QuTech and Kavli Institute of Nanoscience, Delft University of Technology, P.O. Box 5046, 2600 GA Delft, The Netherlands}
\affiliation{Present address: AWS Center for Quantum Computing, 290 South Holliston Avenue, California Institute of Technology, Pasadena, CA 91106 USA}

\author{M.~W.~Beekman}
\affiliation{QuTech and Kavli Institute of Nanoscience, Delft University of Technology, P.O. Box 5046, 2600 GA Delft, The Netherlands}
\affiliation{Netherlands Organisation for Applied Scientific Research (TNO), P.O. Box 96864, 2509 JG The Hague, The Netherlands}

\author{N.~Haider}
\affiliation{QuTech and Faculty of Electrical Engineering, Mathematics, and Computer Science, Delft University of Technology, Mekelweg 4, 2628 CD Delft, The Netherlands}

\author{M.~S.~Moreira}
\affiliation{QuTech and Kavli Institute of Nanoscience, Delft University of Technology, P.O. Box 5046, 2600 GA Delft, The Netherlands}
\affiliation{Present address: Department of Electrical Engineering and Computer Science, Massachusetts Institute of Technology, Cambridge, MA 02139, USA}

\author{J.~F.~Marques}
\affiliation{QuTech and Kavli Institute of Nanoscience, Delft University of Technology, P.O. Box 5046, 2600 GA Delft, The Netherlands}
\affiliation{Present address: AWS Center for Quantum Computing, 290 South Holliston Avenue, California Institute of Technology, Pasadena, CA 91106 USA}

\author{B.~Segers}
\affiliation{QuTech and Kavli Institute of Nanoscience, Delft University of Technology, P.O. Box 5046, 2600 GA Delft, The Netherlands}
\affiliation{Present address: Quantware B.V., Elektronicaweg 10, 2628 XG Delft, The Netherlands}

\author{S.~Vallés-Sanclemente}
\affiliation{QuTech and Kavli Institute of Nanoscience, Delft University of Technology, P.O. Box 5046, 2600 GA Delft, The Netherlands}

\author{L.~DiCarlo}
\email{Corresponding author: l.dicarlo@tudelft.nl}
\affiliation{QuTech and Kavli Institute of Nanoscience, Delft University of Technology, P.O. Box 5046, 2600 GA Delft, The Netherlands}


==> Uploaded/sections/preamble.tex <==
\usepackage{lipsum}
\usepackage{float}
\usepackage{tabularx}
\usepackage{upgreek}
%\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{physics}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage[left=23mm,right=13mm,top=35mm,columnsep=15pt]{geometry}
\usepackage{adjustbox}
\usepackage{placeins}
\usepackage[T1]{fontenc}
\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage{csquotes}
\usepackage[mathscr]{eucal} % used for scripted S symbol
\usepackage[globalcitecopy]{bibunits} % for multiple bibliographies
\usepackage[pdftex, pdftitle={Article}, pdfauthor={Author}]{hyperref} % For hyperlinks in the PDF
\usepackage[capitalize]{cleveref}
\usepackage{multirow}
\usepackage{siunitx}
\usepackage{natbib}

